Trajectory tracking with an aggregation of domestic hot water heaters: Combining model-based and model-free control in a commercial deployment

Scalable demand response of residential electric loads has been a timely research topic in recent years. The commercial coming of age or residential demand response requires a scalable control architecture that is both efficient and practical to use. This work presents such a strategy for domestic hot water heaters and present a commercial proof-of-concept deployment. The strategy combines state of the art in aggregate-and-dispatch with a novel dispatch strategy leveraging recent developments in reinforcement learning and is tested in a hardware-in-the-loop simulation environment. The results are promising and present how model-based and model-free control strategies can be merged to obtain a mature and commercially viable control strategy for residential demand response.

==> sy-headinput.tex <==
% Modified .tex file
%--------------------------------------------------------
%\makeindex
%\pagenumbering{roman}
%\tableofcontents
%\listoffigures
%\listoftables
%---------------------------------
%\input setwmf
%\input seteps
%\begin{figure}[hbtp]
%\centerwmf{6in}{4in}{}
%\caption{Open-loop simulink structure}
%\label{yyy}
%\end{figure}
%See Fig.~\ref{yyy}
%=========================================================
%       Definitions                                 %
% Latex abbrevs ----------------------------------------

\newcommand{\0}{{\bf 0}}


\newcommand{\ba}{\begin{array}}
\newcommand{\ea}{\end{array}}
\newcommand{\bc}{\begin{center}}
\newcommand{\ec}{\end{center}}

\newcommand{\beqn}[1]{\begin{equation}\label{#1}}
\newcommand{\eeqn}{\end{equation}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}

\newcommand{\beqnn}{\begin{eqnarray}}
\newcommand{\eeqnn}{\end{eqnarray}}
\newcommand{\non}{\nonumber}
%-------------------------------------------------------
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}
\newtheorem{definition}{Definition}
\newtheorem{property}{Property}
\newtheorem{proposition}{Proposition}
%-------------------------------------------------------
\newcommand{\va}{\vspace*{5mm}}
\newcommand{\vb}{\vspace*{10mm}}
\newcommand{\vc}{\vspace*{15mm}}
\newcommand{\ha}{\mbox{}\hspace*{5mm}}
\newcommand{\hb}{\mbox{}\hspace*{10mm}}
\newcommand{\hc}{\mbox{}\hspace*{15mm}}

\newcommand{\hsp}{\mbox{}\hspace{8mm}}
%-------------------------------------------------------
\newcommand{\thetat}{{\theta}^{\T}}
\newcommand{\btheta}{\bar{\theta}}
\newcommand{\bthetat}{\bar{\theta}^{\T}}
\newcommand{\htheta}{\hat{\theta}}
\newcommand{\hthetat}{\hat{\theta}^{\T}}
\newcommand{\ttheta}{\tilde{\theta}}
\newcommand{\tthetat}{\tilde{\theta}^{\T}}

\newcommand{\varphit}{\varphi^{\T}}
\newcommand{\hvarphi}{\hat{\varphi}}
\newcommand{\hvarphit}{\hat{\varphi}^{\T}}

\newcommand{\hy}{\hat{y}}
\newcommand{\ty}{\tilde{y}}
\newcommand{\hu}{\hat{u}}
\newcommand{\tu}{\tilde{u}}

\newcommand{\un}[1]{\underline{#1}\,}

%-------------------------------------------------------
\newcommand{\aaa}{{\rm a}}
\newcommand{\ddd}[1]{{\rm d}{#1}}
\newcommand{\eee}[1]{{\rm e}^{#1}}
\newcommand{\e}[1]{{\rm e}^{#1}}
\newcommand{\fff}{{\rm f}}
\newcommand{\jjj}{{\rm j}}

\newcommand{\C}{{\mathbb C}}
\newcommand{\R}{{\mathbb R}}
\newcommand{\RRR}{{\rm R}}
\newcommand{\CCC}{{\rm C}}


\newcommand{\ccc}{{\rm c}}
\newcommand{\co}{{\rm co}}
\newcommand{\ooo}{{\rm o}}
\newcommand{\ob}{{\rm ob}}
%-----------------------------------------
\newcommand{\adj}{{\rm\,adj}}
\newcommand{\AR}{{\rm AR}}
\newcommand{\arctg}{{\rm arctg}}
\newcommand{\asas}{{\rm a.s.}}

\newcommand{\blank}{{\ \ }}

\newcommand{\col}{{\rm col}}
\newcommand{\coeff}{{\rm coeff}}
\newcommand{\const}{{\rm const}}
\newcommand{\cov}{{\rm cov}}
%\newcommand{\def}{{\rm def}}
\newcommand{\diag}{{\rm diag}}

\newcommand{\E}{{\rm E}}

\newcommand{\FFLS}{{\rm FFLS}}
\newcommand{\grad}{{\rm grad}}
\newcommand{\HH}{{\rm H}}

\newcommand{\Ima}{{\rm Im}}

\newcommand{\IV}{{\rm IV}}
\newcommand{\LCM}{{\rm LCM}}
\newcommand{\LS}{{\rm LS}}
\newcommand{\msms}{{\rm m.s.}}
\newcommand{\ns}{{\rm ns}}

\newcommand{\rank}{{\rm rank}}
\newcommand{\Rea}{{\rm Re}}

\newcommand{\sgn}{{\rm sgn}}
\newcommand{\T}{{\rm T}}
%\newcommand{\th}{{\rm th}}
\newcommand{\tg}{{\rm tg}}
\newcommand{\tr}{{\rm tr}}
\newcommand{\var}{{\rm var}}

%\dim \det \exp \gcd

%-------------------------------------------------

% functions
\newcommand{\ejt}{ {\rm e}^{\jjj\theta } }
\newcommand{\ejw}{ {\rm e}^{\jjj\omega } }


%-----------matrices--------------------------------

\newcommand{\vect}[2]{\left[\begin{array}{c} #1 \\  #2 \end{array} \right]}
\newcommand{\vectt}[3]{\left[\begin{array}{c} #1 \\  #2 \\  #3 \end{array}\right]}
\newcommand{\vectf}[4]{\left[\begin{array}{c} #1 \\  #2 \\  #3 \\ #4 \end{array}\right]}
\newcommand{\vectfd}[4]{\left[\begin{array}{c} #1 \\  #2 \\  #3 \\  \vdots \\ #4 \end{array}\right]}

\newcommand{\mtwo}[4]{\left[\begin{array}{cc}#1 & #2 \\  #3 & #4\end{array} \right]}

\newcommand{\tfmat}[4]{\left[ \begin{array}{c|c} #1 & #2 \\  \hline
                                                 #3 & #4 \end{array} \right] }

% New added

\newenvironment{example}[1]
{

\bigskip
~ \hrulefill ~

\noindent {\bf Example #1}
\smallskip
}
{ \noindent

 ~ \hrulefill ~

\bigskip
}


\newcommand{\longunderbrace}[1]{
\underbrace{~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~}_{#1}
}           % 45mm(35spaces) long


%-----------------------------------------------------------------------------------

% figures



%\newenvironment{Anumber}[1] {(A #1 )}
